ML4C: Seeing Causality Through Latent Vicinity

Supervised Causal Learning (SCL) aims to learn causal relations from observational data by accessing previously seen datasets associated with ground truth causal relations. This paper presents a first attempt at addressing a fundamental question: What are the benefits from supervision and how does it benefit? Starting from seeing that SCL is not better than random guessing if the learning target is non-identifiable a priori, we propose a two-phase paradigm for SCL by explicitly considering structure identifiability. Following this paradigm, we tackle the problem of SCL on discrete data and propose ML4C. The core of ML4C is a binary classifier with a novel learning target: it classifies whether an Unshielded Triple (UT) is a v-structure or not. Specifically, starting from an input dataset with the corresponding skeleton provided, ML4C orients each UT once it is classified as a v-structure. These v-structures are together used to construct the final output. To address the fundamental question of SCL, we propose a principled method for ML4C featurization: we exploit the vicinity of a given UT (i.e., the neighbors of UT in skeleton), and derive features by considering the conditional dependencies and structural entanglement within the vicinity. We further prove that ML4C is asymptotically correct. Last but foremost, thorough experiments conducted on benchmark datasets demonstrate that ML4C remarkably outperforms other state-of-the-art algorithms in terms of accuracy, reliability, robustness and tolerance. In summary, ML4C shows promising results on validating the effectiveness of supervision for causal learning. Our codes are publicly available at https://github.com/microsoft/ML4C.

==> sec/7_checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See \cref{sec:conclusion}. ML4C requires skeleton as additional input, thus we put identifying reliable and accurate skeleton from data as future work.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{Details of proofs are in the supplementary material due to page limit.}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{We have included the main functionalities of ML4C, synthetic data generator, and ML4C's training data (include instructions) for reproducibility. Details are in the supplementary material.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{Key information is in content. Details are in the supplementary material.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{We carefully design experiments, by running experiments multiple times, including error bars in report to ensure reproducibility. For instance, Table~\ref{table:transferability} contains error bar information.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{We compare our algorithm with 15 SOTA competitors and we have cite these work properly. We also use open source benchmark for evaluation and we also properly cite the creators.}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{We share new assets, include main functionalities of our algorithm, and our training data. A private URL is provided. See details in the supplementary material.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{Due to page limit, the detailed discussion is available in the supplementary material.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{We double-checked that the data we are using/curating contains no personally identifiable information or offensive content.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> tab/accuracy_full.tex <==
\begin{table*}[t]
  \scriptsize
   \setlength{\tabcolsep}{3.0pt}
   \renewcommand{\arraystretch}{0.4}
  \caption{Full result of Table~\ref{table:accuracy}: on full datasets \& average performance of 5 runs.}
  \label{table:accuracy_full}
\begin{center}
\begin{tabular}{c c c c c c c c c c c c c c c c c c c}
    \toprule
    \multicolumn{2}{c}{\multirow{2}{*}{\makecell{Datasets\\ \#nodes/\#edges}}} &
    \multicolumn{5}{c}{supervised} &
    \multicolumn{9}{c}{unsupervised} &
    \multicolumn{3}{c}{no skeleton input} \\
    \cmidrule(r){3-7} \cmidrule(r){8-16} \cmidrule(r){17-19} & 
      & ML4C  &  Jarfo & D2C & RCC  & NCC  &  PC  & CPC  & MPC  &  GMB  & GES & GS & HC & CDS & GNIP & DGNN & BLIP & GRSP\\
    \midrule

cancer & SHD & \textbf{0.0±0.0} & 4 & 3 & 4 & \textbf{0} & 2 & \textbf{0} & \textbf{0} & \textbf{0} & 3 & \textbf{0} & \textbf{0} & 2 & \textbf{0} & 4 & 4 & 4 \\
5/4 & F1 & \textbf{ 1.0±.00} &  .00 &  .25 &  .00 & \textbf{ 1.0} &  .50 & \textbf{ 1.0} & \textbf{ 1.0} & \textbf{ 1.0} &  .25 & \textbf{ 1.0} & \textbf{ 1.0} &  .50 & \textbf{ 1.0} &  .00 &  .00 &  .00 \\
\cmidrule(r){1-19}
earthquake & SHD & \textbf{0.0±0.0} & 4 & 2 & 4 & \textbf{0} & 2 & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} & 4 & \textbf{0} & \textbf{0} & 4 & 5 & \textbf{0} \\
5/4 & F1 & \textbf{ 1.0±.00} &  .00 &  .50 &  .00 & \textbf{ 1.0} &  .50 & \textbf{ 1.0} & \textbf{ 1.0} & \textbf{ 1.0} & \textbf{ 1.0} & \textbf{ 1.0} &  .00 & \textbf{ 1.0} & \textbf{ 1.0} &  .00 &  .00 & \textbf{ 1.0} \\
\cmidrule(r){1-19}
survey & SHD & 1.0±0.0 & 4 & 5 & 4 & \textbf{0} & \textbf{0} & 1 & 1 & \textbf{0} & 4 & \textbf{0} & 6 & 5 & 6 & 6 & 6 & 6 \\
6/6 & F1 &  .83±.00 &  .50 &  .25 &  .33 & \textbf{ 1.0} & \textbf{ 1.0} &  .83 &  .83 & \textbf{ 1.0} &  .44 & \textbf{ 1.0} &  .00 &  .25 &  .00 &  .00 &  .00 &  .00 \\
\cmidrule(r){1-19}
asia & SHD & \textbf{0.0±0.0} & 5 & 7 & 1 & \textbf{0} & 1 & 3 & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} & \textbf{0} & 2 & \textbf{0} & 16 & 6 & 1 \\
8/8 & F1 & \textbf{ 1.0±.00} &  .33 &  .15 &  .80 & \textbf{ 1.0} &  .80 &  .67 & \textbf{ 1.0} & \textbf{ 1.0} & \textbf{ 1.0} & \textbf{ 1.0} & \textbf{ 1.0} &  .67 & \textbf{ 1.0} &  .20 &  .57 & \textbf{ 1.0} \\
\cmidrule(r){1-19}
sachs & SHD & \textbf{0.0±0.0} & 9 & 11 & 8 & 12 & 13 & \textbf{0} & \textbf{0} & 13 & 14 & 11 & \textbf{0} & 8 & \textbf{0} & 16 & 1 & 8 \\
11/17 & F1 & \textbf{ .00±.00} & \textbf{ .00} & \textbf{ .00} & \textbf{ .00} & \textbf{ .00} & \textbf{ .00} & \textbf{ .00} & \textbf{ .00} & \textbf{ .00} & \textbf{ .00} & \textbf{ .00} & \textbf{ .00} & \textbf{ .00} & \textbf{ .00} & \textbf{ .00} & \textbf{ .00} & \textbf{ .00} \\
\cmidrule(r){1-19}
child & SHD & \textbf{0.0±0.0} & 18 & 16 & 18 & 20 & 22 & 13 & 9 & 20 & 15 & 13 & 13 & 18 & \textbf{0} & 23 & \textbf{0} & \textbf{0} \\
20/25 & F1 & \textbf{ 1.0±.00} &  .24 &  .43 &  .33 &  .12 &  .12 &  .00 &  .74 &  .12 &  .47 &  .59 &  .57 &  .34 & \textbf{ 1.0} &  .25 & \textbf{ 1.0} & \textbf{ 1.0} \\
\cmidrule(r){1-19}
insurance & SHD & \textbf{1.8±1.7} & 41 & 30 & 34 & 28 & 36 & 34 & 21 & 29 & 34 & 28 & 19 & 36 & 11 & 53 & 35 & 14 \\
27/52 & F1 & \textbf{ .95±.04} &  .26 &  .44 &  .42 &  .44 &  .39 &  .00 &  .66 &  .55 &  .46 &  .56 &  .76 &  .36 &  .88 &  .05 &  .51 &  .83 \\
\cmidrule(r){1-19}
water & SHD & 8.6±2.6 & 33 & 43 & 31 & \textbf{0} & 4 & 60 & 7 & 8 & 38 & 27 & 38 & 18 & 34 & 61 & 65 & 58 \\
32/66 & F1 &  .90±.03 &  .52 &  .34 &  .56 & \textbf{ 1.0} &  .97 &  .00 &  .91 &  .87 &  .49 &  .62 &  .46 &  .76 &  .57 &  .00 &  .20 &  .21 \\
\cmidrule(r){1-19}
mildew & SHD & 5.6±1.4 & - & 17 & 25 & 34 & 21 & - & - & 7 & \textbf{3} & 9 & 23 & 18 & - & 52 & 36 & 37 \\
35/46 & F1 &  .88±.03 & - &  .68 &  .50 &  .33 &  .56 & - & - &  .85 & \textbf{ .93} &  .80 &  .64 &  .65 & - &  .19 &  .41 &  .47 \\
\cmidrule(r){1-19}
alarm & SHD & \textbf{1.2±0.4} & 21 & 26 & 18 & 20 & 20 & 20 & 6 & 17 & 8 & 3 & 21 & 18 & 2 & 46 & 17 & 2 \\
37/46 & F1 & \textbf{ .97±.01} &  .57 &  .44 &  .64 &  .57 &  .57 &  .57 &  .92 &  .64 &  .86 &  .94 &  .66 &  .62 & \textbf{ .98} &  .12 &  .82 & \textbf{ .98} \\
\cmidrule(r){1-19}
barley & SHD & 3.6±2.4 & 48 & 55 & 50 & \textbf{0} & 3 & - & - & 8 & 42 & - & 34 & 50 & 34 & 87 & 60 & 70 \\
48/84 & F1 &  .97±.02 &  .46 &  .38 &  .44 & \textbf{ 1.0} &  .96 & - & - &  .91 &  .59 & - &  .72 &  .43 &  .74 &  .00 &  .48 &  .45 \\
\cmidrule(r){1-19}
hailfinder & SHD & 11.6±1.0 & 47 & 41 & 43 & \textbf{0} & 17 & - & - & 26 & 60 & - & 59 & 44 & 56 & 76 & 111 & 114 \\
56/66 & F1 &  .79±.03 &  .37 &  .45 &  .42 & \textbf{ 1.0} &  .85 & - & - &  .70 &  .21 & - &  .23 &  .42 &  .32 &  .00 &  .18 &  .15 \\
\cmidrule(r){1-19}
hepar2 & SHD & \textbf{0.0±0.0} & 54 & 81 & 59 & \textbf{0} & 35 & 27 & 37 & 14 & 46 & 40 & 35 & 75 & 48 & 123 & 79 & 64 \\
70/123 & F1 & \textbf{ 1.0±.00} &  .59 &  .34 &  .54 & \textbf{ 1.0} &  .72 &  .81 &  .70 &  .89 &  .75 &  .70 &  .81 &  .39 &  .72 &  .00 &  .54 &  .63 \\
\cmidrule(r){1-19}
win95pts & SHD & 2.0±1.5 & 65 & 51 & 33 & \textbf{0} & 8 & 42 & 7 & 5 & 32 & 21 & 16 & 50 & 27 & 112 & 103 & 23 \\
76/112 & F1 &  .98±.01 &  .43 &  .54 &  .73 & \textbf{ 1.0} &  .95 &  .64 &  .95 &  .97 &  .77 &  .85 &  .91 &  .57 &  .81 &  .00 &  .47 &  .88 \\
\cmidrule(r){1-19}
pathfinder & SHD & 6.8±7.2 & 157 & 145 & 151 & \textbf{0} & 150 & - & - & 147 & 158 & - & 168 & 148 & 119 & 196 & 241 & - \\
109/195 & F1 &  .93±.06 &  .21 &  .29 &  .21 & \textbf{ 1.0} &  .29 & - & - &  .30 &  .29 & - &  .28 &  .31 &  .00 &  .00 &  .07 & - \\
\cmidrule(r){1-19}
munin1 & SHD & \textbf{11.8±1.8} & 169 & 154 & 153 & 72 & 86 & 117 & - & 84 & 109 & - & 233 & 151 & 265 & - & 257 & - \\
186/273 & F1 & \textbf{ .96±.01} &  .42 &  .47 &  .46 &  .77 &  .71 &  .58 & - &  .72 &  .67 & - &  .26 &  .50 &  .00 & - &  .42 & - \\
\cmidrule(r){1-19}
andes & SHD & \textbf{0.6±0.8} & 226 & 209 & 246 & \textbf{0} & 4 & 83 & 4 & 5 & 47 & 15 & 38 & 149 & 328 & - & 175 & 146 \\
223/338 & F1 & \textbf{ 1.0±.00} &  .35 &  .41 &  .29 & \textbf{ 1.0} &  .99 &  .75 &  .99 &  .98 &  .92 &  .96 &  .92 &  .60 &  .00 & - &  .76 &  .75 \\
\cmidrule(r){1-19}
diabetes & SHD & 37.6±4.9 & 220 & 395 & 237 & 48 & \textbf{0} & - & - & 204 & 146 & - & 592 & 368 & - & - & 534 & - \\
413/602 & F1 &  .94±.01 &  .62 &  .38 &  .62 &  .96 & \textbf{ 1.0} & - & - &  .68 &  .77 & - &  .03 &  .43 & - & - &  .43 & - \\
\cmidrule(r){1-19}
pigs & SHD & \textbf{0.0±0.0} & 350 & 332 & 263 & 400 & 400 & - & - & 268 & \textbf{0} & - & 532 & 316 & - & - & 6 & - \\
441/592 & F1 & \textbf{ 1.0±.00} &  .44 &  .46 &  .59 &  .35 &  .35 & - & - &  .56 & \textbf{ 1.0} & - &  .18 &  .50 & - & - & \textbf{ 1.0} & - \\
\cmidrule(r){1-19}
link & SHD & \textbf{1.6±1.6} & 731 & 630 & 638 & 749 & 737 & - & - & 204 & 324 & - & 1047 & 400 & - & - & 947 & - \\
724/1125 & F1 & \textbf{ 1.0±.00} &  .38 &  .45 &  .45 &  .39 &  .40 & - & - &  .81 &  .80 & - &  .14 &  .64 & - & - &  .49 & - \\
\cmidrule(r){1-19}
munin & SHD & 69.2±7.4 & 967 & 790 & 816 & \textbf{0} & 156 & - & - & 458 & 661 & - & 1397 & 795 & - & - & 1599 & - \\
1041/1397 & F1 &  .95±.00 &  .36 &  .48 &  .44 & \textbf{ 1.0} &  .89 & - & - &  .69 &  .62 & - &  .00 &  .51 & - & - &  .29 & - \\
\cmidrule(r){1-19}
munin2 & SHD & \textbf{114.6±27.5} & 554 & 611 & 646 & 1052 & 898 & - & - & 536 & 632 & - & 1240 & 753 & - & - & 1321 & - \\
1003/1244 & F1 & \textbf{ .92±.02} &  .60 &  .56 &  .55 &  .19 &  .30 & - & - &  .57 &  .58 & - &  .01 &  .49 & - & - &  .46 & - \\
\cmidrule(r){1-19}
munin3 & SHD & \textbf{104.6±26.2} & 616 & 629 & 688 & 1048 & 860 & - & - & 544 & 566 & - & 1306 & 819 & - & - & 1539 & - \\
1041/1306 & F1 & \textbf{ .93±.02} &  .58 &  .57 &  .54 &  .25 &  .37 & - & - &  .60 &  .65 & - &  .00 &  .46 & - & - &  .26 & - \\
\cmidrule(r){1-19}
munin4 & SHD & \textbf{95.8±21.7} & 696 & 658 & 776 & 1058 & 876 & - & - & 649 & 618 & - & 1388 & 812 & - & - & 1627 & - \\
1038/1388 & F1 & \textbf{ .94±.01} &  .54 &  .56 &  .50 &  .29 &  .39 & - & - &  .55 &  .64 & - &  .00 &  .49 & - & - &  .28 & - \\
\midrule
\multirow{2}{*}{rank(SHD)} & mean & \textbf{1.7} & 10.0 & 9.4 & 8.7 & 4.8 & 7.0 & 9.8 & 8.2 & 4.3 & 6.5 & 8.5 & 8.3 & 8.3 & 8.1 & 14.2 & 11.4 & 10.2 \\
 & $\pm$stdd & \textbf{1.1} & 3.5 & 3.9 & 2.6 & 4.5 & 4.2 & 4.5 & 5.1 & 3.4 & 4.0 & 4.7 & 3.8 & 3.1 & 5.1 & 2.2 & 3.8 & 4.2\\
\midrule
\multirow{2}{*}{UT-F1} & mean & \textbf{.90} & .22 & .19 & .27 & .66 & .50 & .53 & .87 & .59 & .54 & .77 & .47 & .30 & .55 & .09 & .36 & .55 \\
 & $\pm$stdd & \textbf{.13} & .17 & .13 & .18 & .40 & .34 & .33 & .16 & .32 & .28 & .24 & .35 & .22 & .07 & .42 & .29 & .38 \\
    \bottomrule
  \end{tabular} 
  \end{center}
  \vspace{-1em}
\end{table*}
